Letter of intent for ALICE 3: A next-generation heavy-ion experiment at the LHC

This document describes the plans of the ALICE Collaboration for a major upgrade of its detector, referred to as ALICE 3, which is proposed for physics data-taking in the LHC Run 5 and beyond. ALICE 3 will enable an extensive programme to fully exploit the LHC for the study of the properties of strongly interacting matter with high-energy nuclear collisions. The proposed detector layout, based on advanced silicon sensors, features superb pointing resolution, excellent tracking and particle identification over a large acceptance and high readout-rate capabilities. This document discusses the proposed physics programme, the detector concept, and its physics performance for a suite of benchmark measurements.

==> performance/detector_performance/detector_performance_electron_identification_o.tex <==
\subsubsection{Electron identification}
\label{sec:performance:detector:electron_id}



In this section we consider a magnetic field in the solenoid of \SI{0.5}{\tesla}. Further studies for other magnetic field configurations are under way.
For measurements of thermal dilepton emission, high-purity electron identification at low transverse momentum is required. With the $B=0.5$ T field configuration, the \InnerTOF can provide electron identification starting from $\pt = 0.015$ \GeVc up to $p = 0.1 \GeVc$. At higher momenta the $\beta$ of pions and muons are close to that of electrons, and they cannot be clearly separated anymore. Electron identification at momenta larger than 0.1 \GeVc is provided by the \OuterTOF, which allows the separation of electrons from the other charged particles up to 0.5 \GeVc. In the same momentum range as the \OuterTOF, the \RICH signals of electrons are well separated from the pion and muon bands, extending the electron identification up to 1 \GeVc.


The combination of the information from different detector systems allows to obtain high electron identification efficiencies over a large momentum range while keeping the hadron contamination at a low level. An example of such a combination, this time including an estimate of the tracking efficiency, is shown in \Fig{fig:performance:dectector:electon_id:contamination_and_eff} for the \OuterTOF and the \RICH.

\begin{figure}
  \centering
  \includegraphics[width=.49\textwidth]{performance/figures/electronID/effdiffscenarios_b0.5_0}
  \includegraphics[width=.49\textwidth]{performance/figures/electronID/contamiantion_pt_b0.5}
  \caption[Electron efficiency and contamination] {
    Left: track efficiency of electrons and positrons as a function of \pt, considering different PID scenarios in a magnetic field of 0.5 T.
    In blue circles, using only a TOF detector and in red squares, yellow diamonds and green crosses, using a TOF and RICH detector with a 3.0, 3.5 and 4.0 \richsigma{\pi} rejection cut.
    Right: separation of contamination contributions as a function of \pt, using a TOF+RICH scenario with a 4.0 \richsigma{\pi} rejection cut in a magnetic field of B = 0.5 T.
    In black the total contamination, in blue the contamination from muons and in red the contamination from pions is shown.
    No mismatch was considered in these projections.
  }
  \label{fig:performance:dectector:electon_id:contamination_and_eff}
\end{figure}

The efficiency obtained by applying a selection of electrons with $\tofNsigma{e} < 3$ is shown as a function of \pt in \Fig{fig:performance:dectector:electon_id:contamination_and_eff} (left) for different rejection criteria on the pions.
The contamination, corresponding to a selection of $\richNsigma{\pi} < 4$ is shown in \Fig{fig:performance:dectector:electon_id:contamination_and_eff} (right).
In the region with sufficient efficiency for a measurement, below $\pt = 2$ \GeVc, the contamination is found to be below 5\%.
The $4\sigma$ rejection translates to a rejection factor of $10^5$ for the pions and $10^2$ for the muons.

At high \pt, the ECAL can be used to identify electrons with the $E/p$ method. This method generally provides sufficient purity to measure decays of quarkonia and open heavy-flavour hadrons, while the misidentification background may be too large for measurements of the thermal continuum.











==> performance/detector_performance/detector_performance_hadron_identification_o.tex <==
\subsubsection{Hadron identification}
\label{sec:performance:detector:hadron_id}

\begin{figure}[tbp] %
  \centering
  \includegraphics[width=\textwidth]{performance/figures/hadron_identification/ngPID_fwd_B05T.pdf}
  \caption[Particle identification (analytical, \SI{0.5}{\tesla})]{
    Analytical calculations of the $\eta-\pt$ regions in which particles can be separated by at least $3\sigma$ for the ALICE 3 particle-identification subsystems embedded in a 0.5~T magnetic field. Electron/pion, pion/kaon and kaon/proton separation plots are shown from left to right.
  }
    \label{fig:performance:detector:hadron_id:summary:5kgauss}
 \includegraphics[width=\textwidth]{performance/figures/hadron_identification/ngPID_fwd_2T.pt.pdf}
  \caption[Particle identification (analytical, \SI{2}{\tesla})]{
    Analytical calculations of the $\eta-\pt$ regions in which particles can be separated by at least $3\sigma$ for the ALICE 3 particle-identification systems embedded in a 2.0~T magnetic field. Electron/pion, pion/kaon and kaon/proton separation plots are shown from left to right.
  }
  \label{fig:performance:detector:hadron_id:summary:2tesla}
\end{figure}

Hadron identification in the central barrel detector and in the forward region is performed via time-of-flight and Cherenkov imaging techniques. Figure~\ref{fig:performance:detector:hadron_id:summary:5kgauss} and~\ref{fig:performance:detector:hadron_id:summary:2tesla} summarise the PID capabilities of the proposed detector, highlighting the $\eta-\pt$ regions where particle identification with a better than 3$\sigma$ separation is possible. It is worth noticing the expected larger low-\pt acceptance in the B = 0.5 T field configuration when compared to the 2 T case, however it is important to note that effects due to interaction of particles with the detector material are not taken into account in this study.

Two layers of time-of-flight detectors, \InnerTOF and \OuterTOF, are located at 20~cm and 105~cm from the beam pipe and measure the arrival time of particles with a resolution of 20~ps. Forward TOF walls with the same time resolution are located at 405~cm on either side of the interaction point.
A description of the implementation and technology for the TOF systems is given in detail in Section~\ref{sec:systems:tof}.
The start time is self-determined by the system of time-of-flight detectors with a resolution better than 3~ps in high-multiplicity events, which adds a negligible contribution to the time-of-flight measurement.
\new{It should be noted that the combination of bTOF1 and bTOF2 also allows the true measurement of the time of flight and, thus, also the precise determination of the start time even with few tracks.}
The length of the track is measured by the tracking system and its resolution is assumed to be negligible.

Figure~\ref{fig:performance:detector:hadron_id:tof2:beta} shows the response of the barrel TOF systems for simulated \PbPb{} events in a magnetic field of $B = \SI{2}{T}$. 
It can be seen that due to the larger occupancy, the fake hit association is larger for the \InnerTOF layer, causing an increase in the background due to track-TOF mismatch. 

\begin{figure} %
  \centering
  \includegraphics[width=0.47\textwidth]{performance/figures/hadron_identification/beta_innerTOF_PbPb_B2T}\hfill%
  \includegraphics[width=0.47\textwidth]{performance/figures/hadron_identification/beta_outerTOF_PbPb_B2T}
  \caption[Particle velocity from inner and outer TOF] {
    Momentum dependent distribution of the particle velocity measured with the \InnerTOF (left) and \OuterTOF (right) in \PbPb collisions with the B~=~\SI{2}{T} configuration.
    The momentum thresholds for the different particle species are clearly visible for the two detector configurations as well as the effect of the improved momentum resolution.
  }
  \label{fig:performance:detector:hadron_id:tof2:beta}
\end{figure}



The barrel RICH detector, \RICH, is composed of a 2~cm thick aerogel radiator with refractive index $n = 1.03$ located at 110~cm from the beam line and followed by a 20 cm expansion volume with photo-detector readout.
Such a system is expected to provide a measurement of the Cherenkov angle with an average angular resolution of 1.5~mrad. 
For the forward region, RICH detectors with the matching performance but smaller refractive index are assumed at a longitudinal distance of 410~cm on either side of the interaction point.
This is still subject to optimisation.

\begin{figure}[tbp] %
  \centering
  \includegraphics[width=0.45\textwidth]{performance/figures/hadron_identification/angle_RICH_PbPb_2T}
  \caption[Cherenkov angle from the barrel RICH] {
    Momentum dependent distribution of the Cherenkov angle measured with the aerogel-based barrel RICH in \PbPb collisions.
    The momentum thresholds for the different particle species are clearly visible. 
    This is the combined result of the effect of the magnetic field and intrinsic threshold for the emission of Cherenkov light in the radiator.
  }
  \label{fig:performance:detector:hadron_id:rich:angle}
\end{figure}

The performance of the \RICH detector is reported in \Fig{fig:performance:detector:hadron_id:rich:angle}, where the measured Cherenkov angle is shown as a function of the reconstructed track momentum.
As for the TOF systems, the identification thresholds of the different particle species can be seen. In this case, the Cherenkov emission threshold determines the low-momentum cut-off for particle identification.







\begin{figure} %
  \centering
  \includegraphics[width=0.46\textwidth]{performance/figures/hadron_identification/Pi_all_det}
  \includegraphics[width=0.46\textwidth]{performance/figures/hadron_identification/Ka_all_det}
  \includegraphics[width=0.46\textwidth]{performance/figures/hadron_identification/Pr_all_det}
  \caption[PID purity] {
  Purity of pions, kaons and protons obtained with the \InnerTOF, \OuterTOF and \RICH in \PbPb collisions with a $3\sigma$ cut with the $B = \SI{2}{\tesla}$ configuration.
  }
  \label{fig:performance:detector:hadron_id:tof:inner_separation_purity}
\end{figure}

Figure~\ref{fig:performance:detector:hadron_id:tof:inner_separation_purity} shows the selection purity with a $3\sigma$ cut on each particle hypothesis, i.e. keeping the PID efficiency above 99\%, for the three different identification systems.


 





\begin{figure}[t] %
  \centering
  \includegraphics[width=.45\textwidth]{performance/figures/nuclei_and_hypernuclei/cls_distribution_sim}
  \caption[Cluster sizes for $z=1$ and $z=2$ particles]{
    Cluster size distribution for $z=1$ and $z=2$ charged nuclei with momenta corresponding to minimum ionizing particles obtained from Monte Carlo simulations of the ALPIDE chip.
  }
  \label{fig:performance:detector:nuclei:clustersize}
\end{figure}

The identification of light nuclei will be mostly based on the TOF measurement. The measurement
allows the distinction of light nuclei with different $m/z$, leaving a residual ambiguity for nuclei sharing the same $m/z$ (e.g. triton and \hesix).
Given the very large differences in the production yields of nuclei with same $m/z$, it is imperative to resolve this ambiguity. This calls for a charge-sensitive measurement.
The feasibility of such a separation has been studied based on the cluster-size of the hits in the tracking layers.
While the details of the response of the tracking layer chips for \ALICETHR are still subject to optimisation (see Section~\ref{sec:systems:tracking} for details), for this study, we employed the simulation of the ALPIDE chip implemented in the O2 framework, as a proof of concept.
The probability distributions of the cluster size corresponding to particles with $z=1$ (protons) and $z=2$ (\hethree) is shown in Fig.~\ref{fig:performance:detector:nuclei:clustersize} for momenta that correspond to minimum ionizing particles.
The distribution for \hethree is shifted towards larger cluster sizes as expected from the $z^{2}$ dependence of the energy loss in the material.
The average cluster size distribution expected when sampling from this distribution over all the tracking layers should therefore allow some separation between the two particles.
While the effectiveness of these considerations clearly depends on the final implementation of the detector, it can be taken as a proof of concept and further developed for the final detector, possibly with the usage of neural network algorithms.



==> performance/detector_performance/detector_performance_muon_identification_o.tex <==
\subsubsection{Muon identification}
\label{sec:performance:detector:muon_id}


Muon identification in ALICE~3 is based on the matching of the information from the tracker and the muon identifier. 
The design of the muon identifier is described in Section~\ref{sec:systems:muon}.
The thickness profile of the hadron absorber has been designed with the goal of achieving enough ($\gtrsim 20\,\%)$ acceptance down to $\pt = 0$ for dimuon invariant masses of $M_{\mu\mu} \approx 3$~GeV/$c^2$, in the whole rapidity region $\abs{\eta} < 1.5$ covered by the detector. %


The muon identification strategy starts with the reconstruction of tracklets in the muon identifier: a tracklet is defined as a straight segment connecting a pair of space points in the two detector layers. Some basic selection criteria on the orientation of the tracklets are imposed, under the hypothesis of particles coming from the interaction region, in order to reject a large fraction of the tracklets built out of combinations of uncorrelated space points. These cuts are optimized with the help of Monte Carlo simulations, with the goal of minimizing the loss of reconstruction efficiency for good tracklets.

The matching between the information of the internal tracker and the muon identifier is then performed by extrapolating each track to the innermost layer of the muon identifier system, taking into account the effect of the magnetic field and the energy loss in the traversed materials. The extrapolated track is then compared with the available tracklets. Only tracklets falling within a search window defined around the extrapolated tracks are considered as valid candidates for the definition of a ``global'' track. The size of the search region is optimized with the help of Monte Carlo simulations, with the goal of minimizing the loss of reconstruction efficiency for good global tracks, where the information from the inner tracker and the muon identifier corresponds to the same particle. Whenever more than one compatible tracklet is found within the search window, a global track is built out of each of them, and the one corresponding to the best global fitting $\chi^2$ is retained. The default strategy for the definition of the global fitting $\chi^2$ is based on a Kalman filter approach, combining the space points reconstructed in the inner tracking system and the muon identifier. 
Alternative criteria for the selection of the best global track candidate are under study.

By definition, a global track (a track from the inner tracker having found at least one valid extrapolation in the muon identifier) is identified as a muon track. The performance of the muon identification system was studied with GEANT4 simulations of pp events and the muon efficiency and hadron rejection factors were determined and parametrised for use in \delphesotwo. It was verified that the occupancy in \PbPb simulations is small enough that the expected impact on the performance is negligible. The efficiency and contamination from fast simulation is shown in Fig.~\ref{fig:performance:dectector:muonID:kineBeforeAfterMID} for muons, pions, and kaons, and the MID is found to be nearly $100\,\%$ efficient in identifying muons starting from $\pt \sim 1.5$~GeV/$c$ at $\eta = 0$, providing pion and kaon rejection factors of \numrange{50}{100}. Comparative studies on the physics performance in the muon and electron channels are ongoing.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.55\textwidth]{performance/figures/muonID/AccMuons_1D.pdf}
  \includegraphics[width=0.65\textwidth]{performance/figures/muonID/distru_ratio_MID_3.png}
  \includegraphics[width=0.65\textwidth]{performance/figures/muonID/distru_ratio_MID_4.png}

  \caption[Muon efficiency and contamination] {\comment{Figure needs graphical improvement}MID rejection factor for muons as a function of $\pt$; $\mu/\pi$ ratio and $\mu/$K ratio, before and after MID identification, as a function of $\pt$.}
  \label{fig:performance:dectector:muonID:kineBeforeAfterMID}
\end{figure}

==> performance/detector_performance/detector_performance_o.tex <==
\subsection{Detector performance}
\label{sec:performance:detector}

\begin{revised}
In this section, the expected detector performance based on the detector specifications outlined in Section~\ref{sec:introduction:experimental_layout} is discussed.
The performance studies are based on a parametrisation of the momentum resolution with a solenoid and two dipole magnets, to assess the ultimate physics reach of the experiment. 
The impact of the reduced performance as achieved with a solenoidal magnet alone will be studied to finalise the design of the magnet system.
Some studies, e.g. on the reconstruction of low-mass dielectrons, assume a reduced magnetic field to increase the acceptance at lower transverse momenta. 
This could be accommodated in a dedicated run as done in Run~2.
\end{revised}




\input{performance/detector_performance/detector_performance_tracking_and_vertexing.tex}
\input{performance/detector_performance/detector_performance_hadron_identification.tex}
\input{performance/detector_performance/detector_performance_electron_identification.tex}
\clearpage %
\clearpage %
\input{performance/detector_performance/detector_performance_muon_identification.tex}
\input{performance/detector_performance/detector_performance_photon_identification.tex}



==> performance/detector_performance/detector_performance_photon_identification_o.tex <==
\subsubsection{Performance of the forward conversion tracker}
\label{sec:performance:detector:photon_id}



As discussed in Section~\ref{sec:physics:ultra-soft-photons:low}, access to the physics in the range relevant for testing Low's theorem poses the challenge of detecting photons down to transverse momenta in the MeV range.
At low photon energies, the photon conversion method generally provides a better energy resolution than a calorimeter measurement. However, also with the conversion method, limitations arise for low-energy photons due to interactions and difficulties in the tracking of the electrons and positrons produced at low momenta. 
These limitations become less problematic for photon energies $E_\gamma \gtrsim 50\text{--}100\,\mathrm{MeV}$. Experimentally, a photon measurement in the MeV/c transverse momentum range is therefore only feasible at larger rapidity. The ratio $E_\gamma / p_{T,\gamma} = \cosh \eta_\gamma$ is 10.1, 27.3, and 74.2 for $\eta_\gamma = 3,\,4,\,5$, respectively. As can be readily seen, experimental access to the MeV/c transverse momentum range becomes progressively easier as the photon rapidity is increased.

We have studied a setup in which a photon converts in front of a Forward Conversion Tracker (FCT) which subtends the pseudorapidity range $3 \lesssim \eta \lesssim 5$. The trajectories of the electron and positron are then measured by a sequence of silicon tracking layers whose spacing increases from below a centimeter to several centimeters. This allows us to measure tracks at low transverse momentum from the MeV range up to the GeV range. 
A transverse component of the magnetic field is necessary to provide sufficient momentum resolution.
A possible location of the FCT would be at a distance of about 3.5\,m away from the primary vertex. 

\begin{figure}
\centering
\includegraphics[width=\linewidth]{performance/figures/fct_performance_pa_bfield500mt_target100mupb_nevt100000_geomc1_sigmapos5mu_0.pdf}
\caption[Soft photon performance]{Photon energy resolution (left), pointing resolution (middle), and photon efficiency (right) of the FCT consisting of 11 silicon tracking layers. The GEANT4 simulation was performed for a dipole field of $B = 0.5\,\mathrm{T}$. A position resolution of $\sigma = 5\,\mathrm{\mu m}$ was assumed for the trackers. The tracker thickness was taken to be $50\,\mathrm{\mu m}$.}
\label{fig:fct_performance}
\end{figure}

The energy resolution, pointing resolution, and photon efficiency for such a setup are determined with a GEANT4 simulation with a simplified track momentum reconstruction and shown in Fig.~\ref{fig:fct_performance}. The photon efficiency $\varepsilon$ is dominated by the photon conversion probability in the $100\,\mathrm{\mu m}$ lead converter. The pointing resolution defines how well photon candidates can be constrained to originate from the primary vertex in order to reject background. Below a photon energy of $E_\gamma \approx 50\,\mathrm{MeV}$ both the energy resolution and the pointing resolution deteriorate significantly reflecting the effect of multiple scattering on the resolution on the momentum of the electron and positron tracks. 

In summary, the FCT as discussed in Section~\ref{sec:systems:fct} provides a photon measurement in the range $E_\gamma \gtrsim 50\,\mathrm{MeV}$. To reach transverse momenta below $p_T \lesssim 10~\mathrm{MeV}/c$, a measurement in the forward region up to $\eta \approx 5$ is necessary.


==> performance/detector_performance/detector_performance_tracking_and_vertexing_o.tex <==
\subsubsection{Tracking and vertexing}
\label{sec:performance:detector:track_vtx}











\begin{figure}[p] %
  \centering
     \includegraphics[width=0.49\textwidth]{performance/figures/Introduction/efficiency_tracking_Pt_PbPb_fast_full_B05T_rmin20_GOOD.eps}
     \includegraphics[width=0.49\textwidth]{performance/figures/Introduction/efficiency_tracking_Pt_PbPb_fast_full_B2T_rmin20_GOOD.eps}
   \caption[Tracking efficiencies from fast and full simulation]{Comparison of the tracking efficiency as a function of the transverse momentum obtained with fast and full simulations of minimum bias \PbPb{} collisions, with minimum radius of the tracks $R = 20$ cm for $B = 0.5$~T (left) and $B=2$~T (right).}
  \label{fig:performance:dectector:introduction:full_fast_efficiency_vs_pt_comparison}
\end{figure}

The expected tracking efficiencies for primary pions, kaons, protons and electrons for the proposed layout is shown in Fig.~\ref{fig:performance:dectector:introduction:full_fast_efficiency_vs_pt_comparison}, as a function of the transverse momentum. Particles are required to reach at least the seventh tracking layer, just outside the inner TOF layer, corresponding to a minimal radius $R = \SI{20}{cm}$. 
The performance is shown for both the full and the fast simulation. The agreement between the two is reasonable, except at lower transverse momenta, where the efficiency expected on the basis of the analytical approach is larger than that currently achieved using a preliminary version of the cellular automaton tracking described in Section~\ref{sec:performance:full-simulation} on full simulation events.
\new{Further optimisation of the track finding in the full simulation is ongoing.}

The reconstruction efficiency exhibits mass ordering below 800 MeV/$c$, above which the detector is able to reconstruct any particle species with an efficiency of nearly 100\%. It is worth mentioning that the B = 0.5 T field configuration has a larger acceptance for electrons and pions at low \pt than the B = 2 T field configuration. For the heavier kaons and protons the low momentum efficiency turn on is similar for the two field configurations, being dominated by the interactions (energy loss, multiple scattering) of the particles with the detector material.

\begin{figure} %
\begin{minipage}{0.49\textwidth}
  \centering
     \includegraphics[width=\textwidth]{performance/figures/tracking_and_vertexing/pt_pi.pdf}
     
   \caption[Transverse momentum resolution]{Comparison of the relative transverse momentum resolution for pions as a function of the \pt obtained with the fast analytical tool for $B = \SI{0.5}{\tesla}$ (red) and $B = \SI{2}{\tesla}$ (blue).
   }
  \label{fig:performance:dectector:introduction:full_fast_momentum_resolution_vs_pt_comparison}
\vfill
\end{minipage}\hfill%
\begin{minipage}{0.49\textwidth}
  \centering
    \includegraphics[width=\textwidth]{performance/figures/tracking_and_vertexing/all_spec_pt_vs_eta.pdf}
   \caption[Transverse momentum resolution]{Relative transverse momentum resolution (in \si{\percent}) as a function of the pseudorapidity obtained with FAT for electrons, pions and protons with $\pt = 1$~\GeVc and minimum radius of the tracks R~=~20~cm in a magnetic field B~=~2~T. The continuation from $|\eta| = 2$ out to $|\eta| = 4$ is set to be constant as achievable  with forward dipoles. \comment{Add unit to vertical axis label; this information is now included in the figure before.}}
  \label{fig:performance:dectector:introduction:momentum_resolution_vs_eta_comparison}
\end{minipage}
\end{figure}
Fig.~\ref{fig:performance:dectector:introduction:full_fast_momentum_resolution_vs_pt_comparison} shows the expected transverse momentum resolution for pions as a function of \pt. We have considered a magnetic field of \SI{0.5}{\tesla} and \SI{2}{\tesla}, which results in a relative resolution of \SI{\sim 2.5}{\percent} and \SI{\sim 0.6}{\percent} at midrapidity, respectively. \new{The ideal field for the overall physics programme has yet to be established and the two configurations cover the considered range of performance.}

\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{systems/Figures_tracker/momentum_resolution-2022-03-01}
    \caption[\pt resolution with different magnetic fields]{Momentum resolution for muons of $\pt = \SI{1}{\giga\eVc}$ with different field configurations together with the Delphes parametrisation used for the physics performance studies. The magnet designs are discussed in Sec.~\ref{sec:systems}.}
    \label{fig:perf:bfield}
\end{figure}


The pseudorapidity dependence of the transverse momentum resolution for  electrons, pions, kaons, and protons with $\pt$~=~1~$\GeVc$ in a magnetic field $B = 2.0$~T is shown in Fig.~\ref{fig:performance:dectector:introduction:momentum_resolution_vs_eta_comparison}. It rises from about 0.7\% (0.9\%) in the most central region for electrons and pions (protons) to about 1.1\% (1.15\%) at $|\eta|=2$. It is then assumed to be constant from there on out to $|\eta|=4$. This could be achieved with an appropriate magnet design allowing for a dipole component at large $z$ (see Fig.~\ref{fig:perf:bfield}).
\new{As the detailed plans for the magnet system are still evolving, the assumption of constant performance allows us best to study the impact of the \pt resolution on the physics performance also in the forward region.}


\paragraph{Determination of the primary vertex position} 

\begin{figure} %
  \centering
    \includegraphics[width=0.7\textwidth]{performance/figures/Introduction/SigmaVtx_together_v1_new_2T_rebin.pdf}
   \caption[Primary vertex resolution]{Resolution of the primary vertex reconstruction in the transverse plane and along the beam axis as a function of the number of contributors to the primary vertex for $B = \SI{2}{\tesla}$.}
  \label{fig:performance:dectector:introduction:primary_vertexing}
\end{figure}

Figure~\ref{fig:performance:dectector:introduction:primary_vertexing} shows the primary vertex resolution of the detector. 
The close proximity of the silicon layers 
to the primary interaction vertex allows the reconstruction of the primary vertex to better than \SI{10}{\micro\metre}.
For this study, primary vertices are determined using 
a track distance minimization procedure
that follows the same algorithm that is currently employed 
in ALICE, based on the performance for primary track reconstruction discussed before. The difference between the vertex position resolution in pp and \PbPb{} collisions at equal multiplicity is due to a different momentum distribution of the particles in the generated events.










The impact parameter resolution along the longitudinal and the transverse directions, evaluated with the fast simulation, is shown in Fig.~\ref{fig:performance:dectector:tracking:dcaxyz} for charged tracks in pp collisions with $B = 2$~T. It is evaluated including the resolution for the reconstruction of the primary vertex position discussed above. Notably, it is observed
to be approximately a factor of five better than the ITS3+TPC 
combination for particles with \pt of \SI{\sim 500}{\mega\eVc}~\cite{ALICE:ITS3:2019}. 

\begin{figure} %
  \centering
  \includegraphics[width=.49\textwidth]{performance/figures/Introduction/RPhiPointingResolutionTOT_pp_2T_eta2_3.eps}
   \includegraphics[width=.49\textwidth]{performance/figures/Introduction/ZPointingResolutionTOT_pp_2T_eta2_3.eps} 
  \caption[Impact parameter resolution]{ 
    The impact parameter resolution for a magnetic field $B = \SI{2}{T}$ in the transverse (longitudinal) direction is shown in the left (right) panel. %
  }
  \label{fig:performance:dectector:tracking:dcaxyz}
\end{figure}

\paragraph{Secondary vertexing}

The secondary vertex position is determined employing track-distance minimisation methods. 
The residuals of the secondary vertex position distributions along the $x$, $y$ and $z$ coordinates are reported in Fig.~\ref{fig:performance:dectector:introduction:secondary_vertexing_resolution_D0_Lc} for two examples: $D^{0}~\to~K^{-}\pi^{+}$ and $\Lambda_{c}^{+}~\to~pK^{-}\pi^{+}$, reconstructed in the transverse momentum interval $1~<~\pt~<~2~\GeVc$. The widths of the distributions are below 5 $\mu$m in all three dimensions for both the $D^{0}$ and $\Lambda_{c}^{+}$ decays.

\begin{figure} %
  \centering
    \includegraphics[width=0.49\textwidth]{performance/figures/Introduction/SecVertex_recoMC_diff_last_D0_1_2_v1_b2T_newvtx.eps}
    \includegraphics[width=0.49\textwidth]{performance/figures/Introduction/SecVertex_recoMC_diff_last_Lc_1_2_v1_b2T_newvtx.eps}
   \caption[Secondary vertex residuals]{Distribution of the secondary vertex residuals for true  $D^{0}~\to~K^{-}\pi^{+}$ and $\Lambda_{c}^{+}~\to~pK^{-}\pi^{+}$ candidates along $x$, $y$ and $z$ direction in the transverse momentum range 1~$<~\pt~<~$2~\GeVc over the full pseudorapidity acceptance $|\eta|<4$ in pp collisions with B~=~2~T.}
  \label{fig:performance:dectector:introduction:secondary_vertexing_resolution_D0_Lc}
\end{figure}




\paragraph{Strangeness tracking}
\label{sec:performance:detector:strangeness_tracking}

\begin{figure} %
  \centering
  \includegraphics[width=.99\textwidth]{performance/figures/tracking_and_vertexing/DecayLengthDist.pdf}
  \caption[Survival probability of $\Xi^{-}$ and $\Omega^{-}$ for strangeness tracking]{
    Survival probability of a $\Xi^{-}$ (magenta line) and $\Omega^{-}$ (blue line) with a momentum of \SI{1}{\giga\eVc} as a function of the distance to the interaction point. The locations of the different layers of the \ALICETHR detector at $\eta=0$ are indicated by the arrows. 
  }
  \label{fig:performance:dectector:tracking:stra_decayLength}
\end{figure}

The ALICE 3 experiment has been designed so that weakly decaying strange particles can be tracked before they decay. 
Figure~\ref{fig:performance:dectector:tracking:stra_decayLength} shows the survival probability of $\Xi^{-}$ and $\Omega^{-}$ baryons with a momentum of 1~\GeVc as a function of the distance to primary vertex. These particles have a probability of at least 90\% and 70\%, respectively, to cross the first layer and leave a direct hit. This method, called `strangeness tracking', decisively improves the reconstruction of weakly decaying particles that stem from multi-charm baryon decays. 

\begin{figure} %
  \centering
  \includegraphics[width=.49\textwidth]{performance/figures/tracking_and_vertexing/StraTrackFullSim.pdf}
  \includegraphics[width=.49\textwidth]{performance/figures/tracking_and_vertexing/StraTrackFullSimZoom.pdf}
  \caption[Illustration of strangeness tracking]{
    (left) Illustration of strangeness tracking from full detector simulation 
    of the $\Xi_{cc}^{++}$ decay into $\Xi_{c}^{+}+\pi^{+}$ with the successive decay $\Xi_{c}^{+}\rightarrow\Xi^{-}+2\pi^{+}$. (right) Close-up illustration of the region marked with a red dashed box in the left figure, containing the 
    five innermost layers of \ALICETHR and the hits that were added to the $\Xi^{-}$ trajectory (red squares).
  }
  \label{fig:performance:dectector:tracking:stratrack}
\end{figure}

Strangeness tracking is implemented as a second stage that follows after 
secondary track finding. The trajectory information of each weak decay candidate 
is calculated and utilized to extrapolate back in the direction of the primary interaction 
vertex. If hits are detected that are sufficiently close to this trajectory, as illustrated 
in Fig.~\ref{fig:performance:dectector:tracking:stratrack}, they 
are added to the track parametrisation, increasing the precision of the
weak decay candidate reconstruction. This increase is mostly related to the position 
of the candidate trajectory, since the momentum information is predominantly acquired 
from the longer daughter tracks. This method provides a much better 
distance-of-closest approach measurement of the weak decay trajectory to the primary 
vertex (see Fig.~\ref{fig:performance:physics:heavy_flav:mcPbPb:DCADemo}), greatly improving the ability to distinguish weak decays from primary or secondary sources. 


An important aspect of strangeness tracking is that the resolution in determining the weak 
decay trajectory has to be sufficiently high to ensure a low fake hit association rate. 
In \ALICETHR, full simulations indicate an average expected occupancy of approximately 10-12 hits per square
millimeter in the innermost layer for central \PbPb{}, corresponding to one hit every
\SI{0.1}{\mm^2}. 
The expected precision of the inwards track propagation results in a search window size of approximately \SI{5e-3}{\mm^2} to be 
used in the innermost layers.
With this method, a impact parameter resolution for multi-strange baryons is achieved, that is similar to that of primary charged particles.

\new{Potential applications of strangeness tracking include the reconstruction of multi-charm and beauty baryons. Performance studies for 
multi-charm baryons are reproduced in Sec.~\ref{sec:performance:physics:heavy_flav:multicharm} and further studies using
this technique will explored in the future.}









